How Developers Iterate on Machine Learning Workflows -- A Survey of the Applied Machine Learning Literature

Machine learning workflow development is anecdotally regarded to be an iterative process of trial-and-error with humans-in-the-loop. However, we are not aware of quantitative evidence corroborating this popular belief. A quantitative characterization of iteration can serve as a benchmark for machine learning workflow development in practice, and can aid the development of human-in-the-loop machine learning systems. To this end, we conduct a small-scale survey of the applied machine learning literature from five distinct application domains. We collect and distill statistics on the role of iteration within machine learning workflow development, and report preliminary trends and insights from our investigation, as a starting point towards this benchmark. Based on our findings, we finally describe desiderata for effective and versatile human-in-the-loop machine learning systems that can cater to users in diverse domains.

==> related.tex <==
%!TEX root=sigconf.tex

To the best of our knowledge, our survey is the first effort in quantitative studies of machine learning model development from empirical evidence.
However, the pursuit of understanding ML development is not singularly ours.
Several surveys have been conducted in recent years to profile industry and academic ML users~\cite{oreilly17, kaggle17, mitreview17}.
These surveys differ from our in nature 
in that they were sent out directly to a select set of industry and academic users.
Many high profile articles discuss general trends in the ML landscape~\cite{domingos2012few, Jordan255, royalsociety17},
while a number of articles focus on 
providing guidance and an ML taxonomy to novice users~\cite{bestPractice, qiu2016survey, gartner17}.
Landset et al. \cite{landset2015survey} surveys open source tools for Big Data machine learning, 
while Vartak et al. \cite{vartak2015supporting} focuses on iterative model building 
and the system desiderata to support this mode of development.

